Constant-Factor Optimization of Quantum Adders on 2D Quantum Architectures

Quantum arithmetic circuits have practical applications in various quantum algorithms. In this paper, we address quantum addition on 2-dimensional nearest-neighbor architectures based on the work presented by Choi and Van Meter (JETC 2012). To this end, we propose new circuit structures for some basic blocks in the adder, and reduce communication overhead by adding concurrency to consecutive blocks and also by parallel execution of expensive Toffoli gates. The proposed optimizations reduce total depth from $140\sqrt n+k_1$ to $92\sqrt n+k_2$ for constants $k_1,k_2$ and affect the computation fidelity considerably.

==> figures/Adder.tex <==
$$
\Qcircuit @C=0.5em @R=0.5em @!R@!C{
\lstick{a_1	}	&\ctrl{1}	&\ctrl{1}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\	
\lstick{b_1	}  	&\ctrl{1}	&\targ	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{0	}  	&\targ	&\qw	&\qswap	&\qw	&\qw	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{a_2	}	&\ctrl{1}	&\ctrl{1}	&\qswap\qwx	&\ctrl{1}	&\ctrl{1}	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{b_2	}	&\ctrl{1}	&\targ	&\qw	&\ctrl{1}	&\targ	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{0	}	&\targ	&\qw	&\qw	&\targ	&\qswap	&\qw	&\qw	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{a_3	}	&\ctrl{1}	&\ctrl{1}	&\qw	&\qw	&\qswap\qwx	&\ctrl{1}	&\ctrl{1}	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{b_3	}	&\ctrl{1}	&\targ	&\qw	&\qw	&\qw	&\ctrl{1}	&\targ	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{0	}	&\targ	&\qw	&\qw	&\qw	&\qw	&\targ	&\qw	&\qw	&\qw	&\qw	&\ctrl{10}	&\qswap	&\qw	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{a_4	}	&\ctrl{1}	&\ctrl{1}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{b_4	}	&\ctrl{1}	&\targ	&\qw	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qswap	&\qw	&\targ	\\
\lstick{0	}	&\targ	&\qw	&\qswap	&\qswap\qwx	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\targ	&\qswap	&\qswap\qwx	&\qswap	&\ctrl{-1}	\\
\lstick{a_5	}	&\ctrl{1}	&\ctrl{1}	&\qswap\qwx	&\ctrl{1}	&\qswap\qwx	&\ctrl{1}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\ctrl{-1}	&\qswap\qwx	&\qswap	&\qswap\qwx	&\qw	\\
\lstick{b_5	}	&\ctrl{1}	&\targ	&\qw	&\ctrl{1}	&\qw	&\ctrl{1}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qswap	&\ctrl{-1}	&\qw	&\qswap\qwx	&\qswap	&\targ	\\
\lstick{0	}	&\targ	&\qw	&\qw	&\targ	&\qswap	&\targ	&\qswap	&\qw	&\qw	&\qswap	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qswap	&\qw	&\qswap\qwx	&\qw	&\qw	&\qw	&\qswap\qwx	&\ctrl{-1}	\\
\lstick{0	}	&\qw	&\qw	&\qw	&\qw	&\qswap\qwx	&\ctrl{1}	&\qswap\qwx	&\qw	&\qswap	&\qswap\qwx	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\targ	&\qw	&\qswap	&\qswap\qwx	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{a_6	}	&\ctrl{1}	&\ctrl{1}	&\qw	&\qswap	&\qw	&\ctrl{1}	&\qw	&\qswap	&\qswap\qwx	&\ctrl{1}	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\ctrl{-1}	&\qswap	&\qswap\qwx	&\qswap	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{b_6	}	&\ctrl{1}	&\targ	&\qw	&\qswap\qwx	&\qswap	&\targ	&\qswap	&\qswap\qwx	&\qw	&\ctrl{1}	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qswap	&\ctrl{-1}	&\qswap\qwx	&\qw	&\qswap\qwx	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\targ	\\
\lstick{0	}	&\targ	&\qw	&\qw	&\qw	&\qswap\qwx	&\qw	&\qswap\qwx	&\qswap	&\qw	&\targ	&\ctrl{1}	&\qw\qwx	&\qswap	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\ctrl{-1}	\\
\lstick{0	}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qswap\qwx	&\qw	&\qw	&\targ	&\qswap\qwx	&\qswap\qwx	&\qswap\qwx	&\ctrl{10}	&\qswap	&\qw	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{a_7	}	&\ctrl{1}	&\ctrl{1}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{b_7	}	&\ctrl{1}	&\targ	&\qw	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qswap	&\qw	&\targ	\\
\lstick{0	}	&\targ	&\qw	&\qswap	&\qswap\qwx	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\targ	&\qswap	&\qswap\qwx	&\qswap	&\ctrl{-1}	\\
\lstick{a_8	}	&\ctrl{1}	&\ctrl{1}	&\qswap\qwx	&\ctrl{1}	&\qswap\qwx	&\ctrl{1}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\ctrl{-1}	&\qswap\qwx	&\qswap	&\qswap\qwx	&\qw	\\
\lstick{b_8	}	&\ctrl{1}	&\targ	&\qw	&\ctrl{1}	&\qw	&\ctrl{1}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qswap	&\ctrl{-1}	&\qw	&\qswap\qwx	&\qswap	&\targ	\\
\lstick{0	}	&\targ	&\qw	&\qw	&\targ	&\qswap	&\targ	&\qswap	&\qw	&\qw	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\qw	&\qw	&\qw	&\qswap	&\qw	&\qswap\qwx	&\qw	&\qw	&\qw	&\qswap\qwx	&\ctrl{-1}	\\
\lstick{0	}	&\qw	&\qw	&\qw	&\qw	&\qswap\qwx	&\ctrl{1}	&\qswap\qwx	&\qw	&\qswap	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\targ	&\qw	&\qswap	&\qswap\qwx	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{a_9	}	&\ctrl{1}	&\ctrl{1}	&\qw	&\qswap	&\qw	&\ctrl{1}	&\qw	&\qswap	&\qswap\qwx	&\ctrl{1}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qw	&\ctrl{-1}	&\qswap	&\qswap\qwx	&\qswap	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
\lstick{b_9	}	&\ctrl{1}	&\targ	&\qw	&\qswap\qwx	&\qswap	&\targ	&\qswap	&\qswap\qwx	&\qw	&\ctrl{1}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw\qwx	&\qw	&\qw\qwx	&\qswap	&\ctrl{-1}	&\qswap\qwx	&\qw	&\qswap\qwx	&\qswap	&\qw	&\qw	&\qw	&\qw	&\qw	&\targ	\\
\lstick{0	}	&\targ	&\qw	&\qw	&\qw	&\qswap\qwx	&\qw	&\qswap\qwx	&\qswap	&\qw	&\targ	&\qw	&\qw	&\qw	&\qw	&\ctrl{1}	&\qw\qwx	&\qswap	&\qw\qwx	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\ctrl{-1}	\\
\lstick{0	}	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\targ	&\qswap\qwx	&\qswap\qwx	&\qswap\qwx	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	&\qw	\\
} 
$$			 		 										

==> figures/Qbitlayout.tex <==
\scriptsize
\begin{tikzpicture}
\draw[step=0.5cm,color=gray] (-1.5,-5.5) grid (0,0);
\node at (-1.25,-.25) {};
\node at (-1.25,-.75) {};
\node at (-1.25,-1.25) {$a_1$};
\node at (-1.25,-1.75) {$b_1$};
\node at (-1.25,-2.25) {0};
\node at (-1.25,-2.75) {$a_2$};
\node at (-1.25,-3.25) {$b_2$};
\node at (-1.25,-3.75) {0};
\node at (-1.25,-4.25) {$a_3$};
\node at (-1.25,-4.75) {$b_3$};
\node at (-1.25,-5.25) {0};
\node at (-0.75,-.25) {$a_4$};
\node at (-0.75,-.75) {$b_4$};
\node at (-0.75,-1.25) {$0$};
\node at (-0.75,-1.75) {$a_5$};
\node at (-0.75,-2.25) {$b_5$};
\node at (-0.75,-2.75) {$0$};
\node at (-0.75,-3.25) {$0$};
\node at (-0.75,-3.75) {$a_6$};
\node at (-0.75,-4.25) {$b_6$};
\node at (-0.75,-4.75) {$0$};
\node at (-0.75,-5.25) {0};
\node at (-0.25,-.25) {$a_7$};
\node at (-0.25,-.75) {$b_7$};
\node at (-0.25,-1.25) {$0$};
\node at (-0.25,-1.75) {$a_8$};
\node at (-0.25,-2.25) {$b_8$};
\node at (-0.25,-2.75) {$0$};
\node at (-0.25,-3.25) {$0$};
\node at (-0.25,-3.75) {$a_9$};
\node at (-0.25,-4.25) {$b_9$};
\node at (-0.25,-4.75) {$0$};
\node at (-0.25,-5.25) {0};
\end{tikzpicture}
\vspace{2cm}
\begin{tabular}{|l|l|l|}
    \hline
    ~		     & $a_4$                  & $a_7$                  \\ 
    ~		     & $b_4,p_4,s_4$          & $b_7,p_7,s_7$          \\ 
    $a_1$     	 & $0,g_4,c_4$            & $0,g_7,c_7$            \\ 
    $b_1,s_1$ 	 & $a_5$                  & $a_8$                  \\ 
    $0,c_2$   	 & $b_5,p_5,s_5$          & $b_8,p_8,s_8$          \\ 
    $a_2$     	 & $0,g_5,P[4,5],c_4,c_5$ & $0,g_8,P[7,8],c_7,c_8$ \\ 
    $b_2,s_2$ 	 & $0,G[4,5],P[4,5]$      & $0,G[7,8],P[7,8]$      \\ 
    $0,c_3$   	 & $a_6$                  & $a_9$                  \\ 
    $a_3$     	 & $b_6,p_6,s_6$          & $b_9,p_9,s_9$          \\ 
    $b_3,s_3$ 	 & $0,g_6,P[4,6],c_4,c_6$ & $0,g_9,P[7,9],c_7,c_9$ \\ 
    $0,c_4$   	 & $0,c[4,6],c_7$          & $0,c[7,9],c_{10}$         \\        
    \hline
\end{tabular}

